Where Should I Look? Optimised Gaze Control for Whole-Body Collision Avoidance in Dynamic Environments

As robots operate in increasingly complex and dynamic environments, fast motion re-planning has become a widely explored area of research. In a real-world deployment, we often lack the ability to fully observe the environment at all times, giving rise to the challenge of determining how to best perceive the environment given a continuously updated motion plan. We provide the first investigation into a `smart' controller for gaze control with the objective of providing effective perception of the environment for obstacle avoidance and motion planning in dynamic and unknown environments. We detail the novel problem of determining the best head camera behaviour for mobile robots when constrained by a trajectory. Furthermore, we propose a greedy optimisation-based solution that uses a combination of voxelised rewards and motion primitives. We demonstrate that our method outperforms the benchmark methods in 2D and 3D environments, in respect of both the ability to explore the local surroundings, as well as in a superior success rate of finding collision-free trajectories -- our method is shown to provide 7.4x better map exploration while consistently achieving a higher success rate for generating collision-free trajectories. We verify our findings on a physical Toyota Human Support Robot (HSR) using a GPU-accelerated perception framework.

==> bib_comments.tex <==
Maier et. al. present and demonstrate an integrated approach for localization, mapping, and planning in 3D environments using RGB-D cameras \cite{Maier2012}. They use a NAO humanoid robot with a depth camera on top of the humanoid's head; they use a fixed mounted position for the camera with the optical axis facing the floor at a 30 degree angle. The authors claim that this was ``found to be the best compromise between observing the near range for obstacle detection and looking ahead for localization and path planning''.




\cite{Bircher2016} propose a planner that uses a receding horizon ``next–best–view'' methodology to fully explore a bounded 3D space.

\cite{Potthast2014} focus on next-best view estimation in cluttered environments. They use a belief model of the unobserved space to estimate the expected information gain associated with each possible viewpoint.

\cite{Border} Border et al. present a scene-model-free NBV planning approach with a density representation; the density of current measurements is used to detect and explore observed surface boundaries.

\cite{Collander2021} introduce a reinforcement learn-
ing approach which uses a topology-based information gain metric for solving the NBV problem.

In all cases, the objective is to estimate the best viewpoints to move to in order to best observe an object or scene. In the context of motion planning, we aren't concerned with observing the environment for the sake of it, we are concerned with observing the parts of the environment that pose the greatest risk to a planned robot trajectory.

\cite{Krainin2011} explore the next best view problem in the somewhat similar context of how a robot manipulator should grasp and move an object in order to best observe an object with a camera and re-create a model of it. 
